Extending the regime of linear response with synthetic forcings

Transport coefficients, such as the mobility, thermal conductivity and shear viscosity, are quantities of prime interest in statistical physics. At the macroscopic level, transport coefficients relate an external forcing of magnitude $\eta$, with $\eta \ll 1$, acting on the system to an average response expressed through some steady-state flux. In practice, steady-state averages involved in the linear response are computed as time averages over a realization of some stochastic differential equation. Variance reduction techniques are of paramount interest in this context, as the linear response is scaled by a factor of $1/\eta$, leading to large statistical error. One way to limit the increase in the variance is to allow for larger values of $\eta$ by increasing the range of values of the forcing for which the nonlinear part of the response is sufficiently small. In theory, one can add an extra forcing to the physical perturbation of the system, called synthetic forcing, as long as this extra forcing preserves the invariant measure of the reference system. The aim is to find synthetic perturbations allowing to reduce the nonlinear part of the response as much as possible. We present a mathematical framework for quantifying the quality of synthetic forcings, in the context of linear response theory, and discuss various possible choices for them. Our findings are illustrated with numerical results in low-dimensional systems.

==> siamart_220329(2)/SF_macros.tex <==
% Renato's custom stuff:
\usepackage{autonum}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{subcaption}
\usepackage{multirow}
\usepackage{booktabs}

\newcommand{\T}{\mathbb{T}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\eps}{\varepsilon}
\renewcommand{\div}{\operatorname{div}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\e}{\mathrm{e}}
\newcommand{\f}{\mathfrak{f}}
\newcommand{\ind}{\mathbf{1}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\Lx}{\widetilde{\L}_\mathrm{extra}}
\newcommand{\Lp}{\widetilde{\L}_\mathrm{phys}}
\newcommand{\Lt}{\widetilde{\L}}
\newcommand{\Lr}{\L_0}
\renewcommand{\S}{\mathscr{S}}
\newcommand{\bigO}{\mathrm{O}}
\newcommand\dpsi[2]{[\Psi^h_{#1}]_{#2}}
\newcommand\ddpsi[2]{[\partial\Psi^h_{#1}]_{#2}}
\newcommand\dfxn[2]{[#1]_{#2}}
\newcommand\sn[2]{{#1}\times 10^{#2}}
\renewcommand{\geq}{\geqslant}
\renewcommand{\leq}{\leqslant}
\renewcommand{\arraystretch}{1.3}

\usepackage{enumitem}
\setenumerate[1]{label={(\arabic*)}}
\setlist[enumerate]{itemsep=0.75em, topsep=0.75em}

\def\code#1{\texttt{#1}}
\newcommand\red[1]{\textcolor{red}{#1}}

% adapted for this siam format
\newtheorem{assumption}{Assumption}
%\newsiamremark{assumption}{Assumption}
\newsiamremark{example}{Example}


%\usepackage{graphicx,epstopdf} % <- Preamble
%\usepackage[caption=false]{subfig} % <- Preamble
%\begin{figure}[tbhp]
%\centering
%\subfloat[$\epsilon_{\max}=5$]{\label{fig:a}\includegraphics{lexample_fig1}}
%\subfloat[$\epsilon_{\max}=0.5$]{\label{fig:b}\includegraphics{lexample_fig2}}
%\caption{Example figure using external image files.}
%\label{fig:testfig}
%\end{figure}
